CAI: An Open, Bug Bounty-Ready Cybersecurity AI

By 2028 most cybersecurity actions will be autonomous, with humans teleoperating. We present the first classification of autonomy levels in cybersecurity and introduce Cybersecurity AI (CAI), an open-source framework that democratizes advanced security testing through specialized AI agents. Through rigorous empirical evaluation, we demonstrate that CAI consistently outperforms state-of-the-art results in CTF benchmarks, solving challenges across diverse categories with significantly greater efficiency -up to 3,600x faster than humans in specific tasks and averaging 11x faster overall. CAI achieved first place among AI teams and secured a top-20 position worldwide in the "AI vs Human" CTF live Challenge, earning a monetary reward of $750. Based on our results, we argue against LLM-vendor claims about limited security capabilities. Beyond cybersecurity competitions, CAI demonstrates real-world effectiveness, reaching top-30 in Spain and top-500 worldwide on Hack The Box within a week, while dramatically reducing security testing costs by an average of 156x. Our framework transcends theoretical benchmarks by enabling non-professionals to discover significant security bugs (CVSS 4.3-7.5) at rates comparable to experts during bug bounty exercises. By combining modular agent design with seamless tool integration and human oversight (HITL), CAI addresses critical market gaps, offering organizations of all sizes access to AI-powered bug bounty security testing previously available only to well-resourced firms -thereby challenging the oligopolistic ecosystem currently dominated by major bug bounty platforms.

==> diagram/sequence_diagram_aztarna.tex <==
\begin{figure}[htbp]
 \centering
 \tikzset{
  % add this style to all tikzpicture environments
  every picture/.append style={
    % enable scaling of nodes
    % set scale factor
    scale=0.2
  }
}
\begin{sequencediagram}
	\renewcommand\unitfactor{1.8}
	\newinst{Robot}{Robot target}
	\newinst[10.0]{Aztarna}{Security researcher: \texttt{aztarna}}
    \begin{scope}[font = \scriptsize]{ }
    	
    	\begin{sdblock}{Phase 1}{Scan and analyze}
        	%\stepcounter{seqlevel}
    		\begin{call}{Aztarna}{}{Robot}{}
    		\end{call}
	    \end{sdblock}
	
	    \begin{sdblock}{Phase 2} {Footprint}
	        %\stepcounter{seqlevel}
        	\begin{call}{Aztarna}{}{Robot}{}
        	\end{call}
        \end{sdblock}		    

	    \begin{sdblock}{Phase 3} {Fingerprint (outside of the scope)}
	        %\stepcounter{seqlevel}
        	\begin{call}{Aztarna}{}{Robot}{}
        	\end{call}

    	\end{sdblock}	
	          
   \end{scope}
\end{sequencediagram}
 \caption{Sequence diagram of \texttt{aztarna}.}
 \label{fig:aztarna/general}
\end{figure}

==> diagram/sequence_diagram_aztarna_industrialrouters.tex <==
\begin{figure}[htbp]
 \centering
 \tikzset{
  % add this style to all tikzpicture environments
  every picture/.append style={
    % enable scaling of nodes
    % set scale factor
    scale=0.2
  }
}
\begin{sequencediagram}
	\renewcommand\unitfactor{2.0}
	\newinst{Router}{Industrial router target}
	\newinst[15.0]{Aztarna}{Security researcher: \texttt{aztarna}}
    \begin{scope}[font = \scriptsize]{ }
    	\begin{sdblock}{Phase 1}{Scan and identification}
        	\stepcounter{seqlevel}
        	\begin{call}{Aztarna}{HTTP Request}{Robot}{HTTP Response containing headers}
        	\end{call}
	    \end{sdblock}
	    \begin{sdblock}{Phase 2}{Authentication}
	        \stepcounter{seqlevel}
	        \begin{call}
	        {Aztarna}{HTTP Request}{Robot}{HTTP 401 Unauthorized response}
	        \end{call}
	        \begin{call}
	        {Aztarna}{HTTP basic authentication response}{Robot}{HTTP 200 OK Response}
	        \end{call}
	        
	        
	    \end{sdblock}
         
	%\begin{sdblock}{alt}{$S$ chooses TCPROS}	
	%\mess{Subscriber}{Terminate connection}{Publisher}
	%	\begin{call}{Subscriber}{Subscribe}{Aztarna}{}
	%	\end{call}
	%	\stepcounter{seqlevel}
	%	\mess{Aztarna}{False data}{Subscriber}
	%\end{sdblock}
	%\begin{sdblock}{Phase 2b}{$sub$ w"ahlt UDPROS als Transportprotokoll}
	          
   \end{scope}
\end{sequencediagram}
 \label{fig:aztarna/industrial_routers}
 \caption{\texttt{aztarna} performing identification and authentication phases for an industrial router.}
\end{figure}

==> diagram/sequence_diagram_aztarna_ros.tex <==
\begin{figure}[htbp]
 \centering
 \tikzset{
  % add this style to all tikzpicture environments
  every picture/.append style={
    % enable scaling of nodes
    % set scale factor
    scale=0.2
  }
}
\begin{sequencediagram}
	\renewcommand\unitfactor{2.0}
	\newinst{Robot}{Robot target}
	\newinst[15.0]{Aztarna}{Security researcher: \texttt{aztarna}}
    \begin{scope}[font = \scriptsize]{ }
    	\begin{sdblock}{Phase 1}{Scan and analyze}
    	\stepcounter{seqlevel}
		\begin{call}{Aztarna}{Invoke \texttt{getsystemstate()}}{Robot}{Return basic footprint}
		\end{call}
		
	\end{sdblock}
	\begin{sdblock}{Phase 2} {Footprint}	

	\begin{sdblock}{Node 1} {}
    	\begin{call}{Aztarna}{Fetch nodes URI through     \texttt{lookupNodes()}}{Robot}{}
    	\end{call}
        
        \begin{call}{Aztarna}{Fetch list of topics through \texttt{getTopicTypes()}}{Robot}{}
    	\end{call}
    	
	\end{sdblock}

	\begin{sdblock}{Node N} {}
    	\begin{call}{Aztarna}{Fetch nodes URI through     \texttt{lookupNodes()}}{Robot}{}
    	\end{call}
        
        \begin{call}{Aztarna}{Fetch list of topics through \texttt{getTopicTypes()}}{Robot}{}
    	\end{call}
    	
	\end{sdblock}	
         
	%\begin{sdblock}{alt}{$S$ chooses TCPROS}	
	%\mess{Subscriber}{Terminate connection}{Publisher}
	%	\begin{call}{Subscriber}{Subscribe}{Aztarna}{}
	%	\end{call}
	%	\stepcounter{seqlevel}
	%	\mess{Aztarna}{False data}{Subscriber}
	%\end{sdblock}
	%\begin{sdblock}{Phase 2b}{$sub$ w"ahlt UDPROS als Transportprotokoll}
	          
   \end{sdblock}		
   \end{scope}
\end{sequencediagram}
 \caption{Sequence diagram of a \texttt{aztarna} scanning a ROS target.}
 \label{fig:aztarna/ros}
\end{figure}

==> diagram/sequence_diagram_aztarna_sros.tex <==
\begin{figure}[htbp]
 \centering
 \tikzset{
  % add this style to all tikzpicture environments
  every picture/.append style={
    % enable scaling of nodes
    % set scale factor
    scale=0.2
  }
}
\begin{sequencediagram}
	\renewcommand\unitfactor{2.0}
	\newinst{Robot}{Robot target}
	\newinst[15.0]{Aztarna}{Security researcher: \texttt{aztarna}}
    \begin{scope}[font = \scriptsize]{ }
    	\begin{sdblock}{Phase 1}{Scan}
    	\stepcounter{seqlevel}
		\mess{Aztarna}{Client Hello}{Robot}{Server Hello}
	\end{sdblock}
	\begin{sdblock}{Phase 2}{Fingerprinting}
		\mess{Robot}{Server Certificate}{Aztarna}
		\mess{Robot}{Client Certificate Request}{Aztarna}
		\mess{Robot}{Server Hello Done}{Aztarna}
	\end{sdblock}
	\begin{sdblock}{Phase 2}{Close Connection}
		\mess{Aztarna}{Disconnect TCP session}{Robot}
	\end{sdblock}
   \end{scope}
\end{sequencediagram}
 \caption{Sequence diagram of a \texttt{aztarna} performing the scan and fingerprinting phases for SROS.}
 \label{fig:aztarna/sros}
\end{figure}
